Examining the Role of Environment in a Comprehensive Sample of Compact Groups

(Abridged) Compact groups, with their high number densities, small velocity dispersions, and an interstellar medium that has not been fully processed, provide a local analog to conditions of galaxy interactions in the earlier universe. The frequent and prolonged gravitational encounters that occur in compact groups affect the evolution of the constituent galaxies in a myriad of ways, for example gas processing and star formation. Recently, a statistically significant "gap" has been discovered mid-infrared IRAC colorspace of compact group galaxies. This gap is not seen in field samples and is a new example of how the compact group environment may affect the evolution of member galaxies. In order to investigate the origin and nature of this gap, we have compiled a sample of 49 compact groups. We find that a statistically significant deficit of galaxies in this gap region of IRAC colorspace is persistant in this sample, lending support to the hypothesis that the compact group environment inhibits moderate SSFRs. We note a curvature in the colorspace distribution, which is fully consistent with increasing dust temperature as the activity in a galaxy increases. This full sample of 49 compact groups allows us to subdivide the data according to physical properties of the groups. An analysis of these subsamples indicates that neither projected physical diameter nor density show a trend in colorspace within the values represented by this sample. We hypothesize that the apparent lack of a trend is due to the relatively small range of properties in this sample. Thus, the relative influence of stochastic effects becomes dominant. We analyze spectral energy distributions of member galaxies as a function of their location in colorspace and find that galaxies in different regions of MIR colorspace contain dust with varying temperatures and/or PAH emission.

==> KStest.tex <==
\ProvidesFile{KSFull.tex}%
 [2003/12/12 5.2/AAS markup document class]%

%$\log{M_{\ion{H}{1}}}$
\begin{deluxetable}{cccccc}
\tablewidth{0pt}
\tablecaption{Results of Statistical Analysis\label{ksfull}}
\tablehead{
\colhead{Compact Groups vs} &	\colhead{N} &	\colhead{$\mathrm{N}_\mathrm{CGs}$} &	\colhead{D} &	\colhead{$\alpha$} &	\colhead{Consistent?}}% \\
%\colhead{} &	\colhead{(J2000)} &	\colhead{(J2000)} &	\colhead{(Mpc)} &	\colhead{}}
\startdata
Uniform Distribution & \nodata & 174 & 0.30 & $2.0\times10^{-13}$ & reject\\
LVL+SINGS	& 93	& 174	& 0.47	& $3.8\times10^{-12}$	& reject\\
Interacting	& 31	& 78	& 0.41	& $1.6\times10^{-3}$	& reject\\
Coma Center	& 114	& 173	& 0.36	& $6.0\times10^{-8}$	& reject\\
Coma Infall	& 47	& 173	& 0.18	& 0.16			& do not reject
\enddata
\tablecomments{Results of the KS test for the compact group distribution against a model and the comparison samples, unwrapped using the quadratic fit to the compact group distribution. $D$ is the maximum deviation (possible range: 0-1) between the two CDFs, while $\alpha$ gives the probability that the two samples were drawn from the same parent distribution (which depends on the number of galaxies in the two samples, $N$, and $N_\mathrm{CGs}$). Based on $\alpha$, we have determined whether the two samples are consistent.}
\end{deluxetable}

\endinput
%%
%% End of file `hcgtable.tex'.
















==> obsinfo.tex <==
\ProvidesFile{obsinfo.tex}%
 [2003/12/12 5.2/AAS markup document class]%

%$\log{M_{\ion{H}{1}}}$
\begin{deluxetable}{ccccc}
\tablewidth{0pt}
\tablecaption{CG Sample\label{cgtable}}
\tablehead{
\colhead{Group} &	\colhead{R.A.\tablenotemark{a}} &	\colhead{Dec\tablenotemark{a}} &	\colhead{D\tablenotemark{a}} &	\colhead{AOR(s)} \\
\colhead{} &	\colhead{(J2000)} &	\colhead{(J2000)} &	\colhead{(Mpc)} &	\colhead{}}
\startdata
H02 & 00$^\mathrm{h}$31$^\mathrm{m}$30\fs0 & +08\degr25\arcmin52\arcsec & 136.6 & r11249152,r11252224\\
H04 & 00$^\mathrm{h}$34$^\mathrm{m}$15\fs9 & -21\degr26\arcmin48\arcsec & 108.9 & r21926400\\
H07 & 00$^\mathrm{h}$39$^\mathrm{m}$23\fs9 & +00\degr52\arcmin41\arcsec & 56.4 & r11249408,r11252480\\
H15 & 02$^\mathrm{h}$07$^\mathrm{m}$39\fs0 & +02\degr08\arcmin18\arcsec & 90.8 & r26875648,r26880512\\
H16 & 02$^\mathrm{h}$09$^\mathrm{m}$31\fs3 & -10\degr09\arcmin31\arcsec & 52.9 & r11249664,r11252736\\
H19 & 02$^\mathrm{h}$42$^\mathrm{m}$45\fs1 & -12\degr24\arcmin43\arcsec & 57.3 & r11249920\\
H22 & 03$^\mathrm{h}$03$^\mathrm{m}$31\fs3 & -15\degr40\arcmin32\arcsec & 36.1 & r11250176,r11252992\\
H25 & 03$^\mathrm{h}$20$^\mathrm{m}$43\fs7 & -01\degr03\arcmin07\arcsec & 84.5 & r26785904,r26880768\\
H26 & 03$^\mathrm{h}$21$^\mathrm{m}$54\fs2 & -13\degr38\arcmin45\arcsec & 126.9 & r23027712\\
H31 & 05$^\mathrm{h}$01$^\mathrm{m}$38\fs3 & -04\degr15\arcmin25\arcsec & 54.6 & r11250432\\
H33 & 05$^\mathrm{h}$10$^\mathrm{m}$47\fs9 & +18\degr02\arcmin05\arcsec & 105.1 & r23027968\\
H37 & 09$^\mathrm{h}$13$^\mathrm{m}$35\fs6 & +30\degr00\arcmin51\arcsec & 95.5 & r23028224\\
H38 & 09$^\mathrm{h}$27$^\mathrm{m}$38\fs8 & +12\degr16\arcmin51\arcsec & 124.3 & r23026432\\
H40 & 09$^\mathrm{h}$38$^\mathrm{m}$54\fs5 & -04\degr51\arcmin07\arcsec & 96.9 & r23025920\\
H42 & 10$^\mathrm{h}$00$^\mathrm{m}$21\fs8 & -19\degr38\arcmin57\arcsec & 53.3 & r11250688,r11253248\\
H47 & 10$^\mathrm{h}$25$^\mathrm{m}$48\fs4 & +13\degr43\arcmin54\arcsec & 135.9 & r23026688\\
H48 & 10$^\mathrm{h}$37$^\mathrm{m}$45\fs6 & -27\degr04\arcmin50\arcsec & 37.7 & r11250944,r11253504\\
H54 & 11$^\mathrm{h}$29$^\mathrm{m}$15\fs5 & +20\degr35\arcmin06\arcsec & 28.1 & r23027456\\
H56 & 11$^\mathrm{h}$32$^\mathrm{m}$39\fs6 & +52\degr56\arcmin25\arcsec & 116.0 & r23026944\\
H57 & 11$^\mathrm{h}$37$^\mathrm{m}$50\fs5 & +21\degr59\arcmin06\arcsec & 131.7 & r23027200\\
H59 & 11$^\mathrm{h}$48$^\mathrm{m}$26\fs6 & +12\degr42\arcmin40\arcsec & 54.1 & r11251200\\
H61 & 12$^\mathrm{h}$12$^\mathrm{m}$24\fs9 & +29\degr11\arcmin21\arcsec & 52.1 & r11251456\\
H62 & 12$^\mathrm{h}$53$^\mathrm{m}$08\fs1 & -09\degr13\arcmin27\arcsec & 54.9 & r11251712\\
H67 & 13$^\mathrm{h}$49$^\mathrm{m}$03\fs5 & -07\degr12\arcmin20\arcsec & 109.9 & r26876160,r26881024\\
H68 & 13$^\mathrm{h}$53$^\mathrm{m}$40\fs9 & +40\degr19\arcmin07\arcsec & 40.7 & r4483584,r27600128\\
\nodata & \nodata & \nodata & \nodata & r27600384,r27600640\\
H71 & 14$^\mathrm{h}$11$^\mathrm{m}$04\fs6 & +25\degr29\arcmin06\arcsec & 131.8 & r23028736\\
H79 & 15$^\mathrm{h}$59$^\mathrm{m}$11\fs9 & +20\degr45\arcmin31\arcsec & 68.0 & r23028992\\
H90 & 22$^\mathrm{h}$02$^\mathrm{m}$06\fs0 & -31\degr55\arcmin48\arcsec & 32.3 & r11251968,r11253760\\
H91 & 22$^\mathrm{h}$09$^\mathrm{m}$10\fs4 & -27\degr47\arcmin45\arcsec & 99.1 & r26877184,r26881536\\
H92 & 22$^\mathrm{h}$35$^\mathrm{m}$57\fs5 & +33\degr57\arcmin36\arcsec & 88.6 & r6011392\\
H96 & 23$^\mathrm{h}$27$^\mathrm{m}$58\fs3 & +08\degr46\arcmin27\arcsec & 118.5 & r12297728\\
H97 & 23$^\mathrm{h}$47$^\mathrm{m}$22\fs9 & -02\degr19\arcmin34\arcsec & 88.3 & r26877440,r26881792\\
H100 & 00$^\mathrm{h}$01$^\mathrm{m}$20\fs8 & +13\degr07\arcmin57\arcsec & 71.9 & r26877696\\
R04 & 00$^\mathrm{h}$42$^\mathrm{m}$49\fs5 & -23\degr33\arcmin11\arcsec & 89.0 & r12342784\\
R06 & 01$^\mathrm{h}$16$^\mathrm{m}$12\fs4 & +46\degr44\arcmin20\arcsec & 69.1 & r26227712\\
R15 & 01$^\mathrm{h}$52$^\mathrm{m}$41\fs4 & +36\degr08\arcmin46\arcsec & 64.3 & r18646272\\
R17 & 01$^\mathrm{h}$56$^\mathrm{m}$21\fs8 & +05\degr38\arcmin37\arcsec & 75.5 & r18030336\\
R21\tablenotemark{\dagger} & 03$^\mathrm{h}$19$^\mathrm{m}$36\fs6 & +41\degr33\arcmin39\arcsec & 68.7 & r10483456\\
R31 & 09$^\mathrm{h}$17$^\mathrm{m}$26\fs5 & +41\degr57\arcmin18\arcsec & 29.5 & r23113472,r23113728\\
R32 & 09$^\mathrm{h}$19$^\mathrm{m}$50\fs8 & +33\degr46\arcmin17\arcsec & 96.3 & r4438784\\
R34 & 09$^\mathrm{h}$43$^\mathrm{m}$12\fs6 & +31\degr54\arcmin44\arcsec & 25.7 & r4439552,r16300032\\
R38 & 10$^\mathrm{h}$51$^\mathrm{m}$46\fs7 & +32\degr51\arcmin31\arcsec & 27.2 & r16304640\\
R42 & 11$^\mathrm{h}$36$^\mathrm{m}$51\fs3 & +19\degr59\arcmin19\arcsec & 93.5 & r25498880\\
R44\tablenotemark{\dagger} & 11$^\mathrm{h}$44$^\mathrm{m}$00\fs6 & +19\degr56\arcmin44\arcsec & 93.6 & r3858688\\
R64 & 12$^\mathrm{h}$41$^\mathrm{m}$33\fs2 & +26\degr03\arcmin56\arcsec & 73.7 & r10532608\\
R66\tablenotemark{\dagger} & 12$^\mathrm{h}$43$^\mathrm{m}$17\fs9 & +13\degr11\arcmin47\arcsec & 13.9 & r4477440,r18288896\\
R67\tablenotemark{\dagger} & 12$^\mathrm{h}$59$^\mathrm{m}$32\fs8 & +27\degr57\arcmin27\arcsec & 106.4 & r3859456\\
R68\tablenotemark{\dagger} & 13$^\mathrm{h}$00$^\mathrm{m}$10\fs7 & +27\degr58\arcmin17\arcsec & 98.3 & r3859712,r3859968\\
R86 & 23$^\mathrm{h}$38$^\mathrm{m}$34\fs4 & +27\degr01\arcmin24\arcsec & 117.6 & r10926592
\enddata
\tablenotetext{a}{Group RA, Dec and distance (corrected for Virgo+GA+Shapley) taken from NED. The cosmology used was $H_0=73\;{\rm km\,s^{-1}\,Mpc^{-1}}$, $\Omega_{matter}=0.27$, and $\Omega_{vacuum}=0.73$.}
\tablenotetext{\dagger}{RSCGs known to be embedded in larger structures.}
\end{deluxetable}

\endinput
%%
%% End of file `hcgtable.tex'.















